A Forward-secure Efficient Two-factor Authentication Protocol

Two-factor authentication (2FA) schemes that rely on a combination of knowledge factors (e.g., PIN) and device possession have gained popularity. Some of these schemes remain secure even against strong adversaries that (a) observe the traffic between a client and server, and (b) have physical access to the client's device, or its PIN, or breach the server. However, these solutions have several shortcomings; namely, they (i) require a client to remember multiple secret values to prove its identity, (ii) involve several modular exponentiations, and (iii) are in the non-standard random oracle model. In this work, we present a 2FA protocol that resists such a strong adversary while addressing the above shortcomings. Our protocol requires a client to remember only a single secret value/PIN, does not involve any modular exponentiations, and is in a standard model. It is the first one that offers these features without using trusted chipsets. This protocol also imposes up to 40% lower communication overhead than the state-of-the-art solutions do.

==> authentication.tex <==

%!TEX root = main.tex



\begin{figure}
 \centering
 \procedure{Authentication}{%
 \textbf{Client} \< \hspace{0ex} \< \textbf{Server} \\
 \pcln \< \< \VS{\counter} \gets \VS{\counter} + 1 \\ % server-- increment counter
 %
 \pcln \< \<  \VS{\keyt_3}, \VS{\state} \gets \update(\VS{\state}, \VS{\counter})\\% server-- update
 %
  \pcln \< \<  \VS{k_1} \gets \prf_{\VS{\keyt_3}}(\VC{\verifier}) \< \< \\
 %
 \pcln \< \< \VS{\nonce} \stackrel{\$}\leftarrow \bin^\secpar\\  % server--pick a challenge
 %
  \pcln \< \< p= \VS{\nonce} || \VS{\counter} || \VS{\trans} \pclb % server--set plaintext
 %
 \sendmessageleftx[7cm]{6}{(M, t)\leftarrow \enc_{\VS{\keyt_3}}(p) } \\ % server--
 %%%%%. client
  \pcln  \tmp_{\VC{\counter}} \gets \VC{\counter} + 1 \\ % client--increment temp-counter
 %
    \pcln  \tmp_{\VC{\state}} \gets \VC{\state} \\ % client-- set temp state
 %
  \pcln  \VC{\keyt_3}, \tmp_{\VC{\state}} \gets \update(\tmp_{\VC{\state}}, \tmp_{\VC{\counter}})\\ % client-- update
 %
  \pcln (p,b) \gets \mathsf{Dec}_{\VC{\keyt_3}}(M,t) \< \< \\% client-- decrypt
  %
  \pcln \iif b\neq 1,    \text{\ then\ go\ to\ } \ref{enroll:fail} \\ % client-- verify tag
  %
   %\pcln \VM{\nonce}, \VM{\counter} \gets \parse(p, |\VC{\counter}|) \< \< \\ % client parse
  %
  \pcln \text{Parse\ } p \text{\ which\ results\ in\ } \VM{\nonce}, \VM{\counter}, \VM{\trans}  \< \< \\ % client parse
 %
 %\pcln \VM{\nonce}, \VM{\counter}, \VM{\trans} \gets \extract_{\VC{\key}}(M) \< \< \\
 %
 \pcln \pcif \VM{\counter} \le \VC{\counter} \pcthen \pcfail ; \highlightkeyword{goto} \ref{auth:fail} \< \< \\
 \pcln \text{Display \VM{\trans} for user to check} \< \< \\
 \pcln \text{\pcif user rejects \VM{\trans}\pcthen \pcfail ; \highlightkeyword{goto} \ref{auth:fail}} \< \< \\
 %
  % \pcln \VC{\counter} \gets \tmp_{\VC{\counter}}\\ % client --set counter 
 %
  \pcln \VC{\counter} \gets \VM{\counter} \< \< \\
  %
 \pcln  \VC{\state} \gets  \tmp_{\VC{\state}}\\% client-- set state
 %
 \pcln \text{Request \VC{\pin} from user} \< \< \\
 %
 \pcln \VC{\verifier} \gets \prf_{\VC{\salt}}(\VC{\pin}) \< \< \\
%
 \pcln  \VC{\keyt_4}, \VC{\state} \gets \update(\VC{\state}, \VC{\counter}) \< \< \\
  %
 \pcln p'=  \VM{\nonce} \|  \VM{\trans} \| \VC{\verifier}\< \< \\ %client--set plaintext
 %
 \pcln \VC{\mathit{response}} \gets \prf_{\VC{\keyt_4}}(p') \< \< \pclb
 %
 \sendmessagerightx[7cm]{6}{M' = \VC{\mathit{response}}} \\
 \pcln \< \< \VS{\mathit{expected}} \gets \prf_{\VS{\keyt2}}(\VS{\nonce} \| \mathbf{T}_\mathrm{AR} \| \VS{\trans} \| \VS{\verifier}) \\
 \pcln \< \< \pcif M \ne \VS{\mathit{expected}} \pcthen \pcfail ; \highlightkeyword{goto} \ref{auth:fail} \\
 \pcln \label{auth:fail} \text{Discard \VC{\pin}, \VC{\verifier}, \VC{\keyt2} \VM{\nonce}, \VM{\trans}} \< \<  \text{Discard \VS{\keyt2}, \VS{\nonce}, \VS{\trans}} \\
 }
    \caption{Authentication phase of protocol}
    \label{fig:auth}
\end{figure}


==> enrollment.tex <==

%!TEX root = main.tex

\begin{figure}
 \centering
 \procedure{Enrollment}{%
 \textbf{Client} \< \hspace{12ex} \< \textbf{Server} \\
 %%%%%% Server
 \pcln \< \< \VS{\counter} \gets \VS{\counter} + 1 \\
 \pcln \< \< \VS{\keyt_1}, \VS{\state} \gets \update(\VS{\state}, \VS{\counter})\\% update
 %
% \pcln \< \< key_1= H(\VS{\keyt_1}||
 %
 \pcln \< \< \VS{\nonce} \stackrel{\$}\leftarrow \bin^\secpar  \\
 %
 \pcln \< \< p= \VS{\nonce}|| \VS{\counter} \pclb % server- set plaintext
 %
 \sendmessageleftx[7cm]{6}{(M,t) \gets \enc_{\VS{\keyt_1}}(p) } \\% encrypt
 %%%%% Client
   \pcln  \tmp_{\VC{\counter}} \gets \VC{\counter} + 1 \\ % increment temp-counter
 %
    \pcln  \tmp_{\VC{\state}} \gets \VC{\state} \\ % client set temp state
 %
  \pcln  \VC{\keyt_1}, \tmp_{\VC{\state}} \gets \update(\tmp_{\VC{\state}}, \tmp_{\VC{\counter}})\\ % client update
 %
  \pcln (p,b) \gets \mathsf{Dec}_{\VC{\keyt_1}}(M,t) \< \< \\% client decrypt
  %
  \pcln \iif b\neq 1,    \text{\ then\ go\ to\ } \ref{enroll:fail} \\ % client verify tag
  %
   \pcln \VM{\nonce}, \VM{\counter} \gets \parse(p, |\VC{\counter}|) \< \< \\ % client parse
  %
 \pcln  \iif \VM{\counter} \le \VC{\counter}, \text{\ then\ go\ to\ } \ref{enroll:fail} \\ %client check counter
 %
 \pcln \VC{\counter} \gets \VM{\counter}\\ % client set counter 
 %
 \pcln  \VC{\state} \gets  \tmp_{\VC{\state}}\\% client set state
 \pcln \text{Request \VC{\pin} from user} \< \< \\
 %
 \pcln \VC{\verifier} \gets \prf_{\VC{\salt}}(\VC{\pin}) \< \< \\
 %\pcln \VC{\counter} \gets \VM{\counter} \< \< \\ % set the counter
 %
  \pcln  \VC{\counter} \gets \VC{\counter} + 1 \\
 %
 \pcln \VC{\keyt_2},  \VC{\state} \gets \update(\VC{\state}, \VC{\counter}) \< \< \\ % update
 %
 \pcln p'=  \VM{\nonce} || \VC{\verifier}\< \< \pclb %client--set plaintext
 %
 \sendmessagerightx[7cm]{6}{(M',t') \gets \enc_{\VC{\keyt_2}}(p') } \\% encrypt
 %%%%%% Server
 %
  \pcln\< \<   \tmp_{\VS{\counter}} \gets \VS{\counter} + 1 \\ % server-- increment temp-counter
 %
    \pcln\< \<   \tmp_{\VS{\state}} \gets \VS{\state} \\ % server-- set temp state
 %
  %\pcln \< \< \VS{\counter} \gets \VS{\counter} + 1 \\
 %
  \pcln \< \< \VS{\keyt_2}, \tmp_{\VS{\state}} \gets \update(\tmp_{\VS{\state}}, \tmp_{\VS{\counter}})\\%  update
  %
  \pcln\< \< (p',b') \gets \mathsf{Dec}_{\VS{\keyt_2}}(M',t') \< \< \\% server-- decrypt
  %
   \pcln\< \< \iif b'\neq 1,    \text{\ then\ go\ to\ } \ref{enroll:fail} \\ % client-- verify tag
  %
 \pcln \< \<  \VM{\nonce},  \VM{\verifier} \gets \parse(p', | \VS{\verifier}|) \< \< \\
  %
% \pcln \< \< \VM{\nonce}, \VM{\verifier} \gets \extract_{\VS{\keyt1}}(M) \\
 \pcln \< \< \iif \VM{\nonce} \ne \VS{\nonce}, \text{then \ go\ to\ } \ref{enroll:fail} \\
 %
  \pcln\< \< \VS{\counter} \gets \tmp_{\VS{\counter}}\\ % client --set counter 
 %
 \pcln\< \<  \VS{\state} \gets  \tmp_{\VS{\state}}\\% client-- set state
 %
 \pcln \< \< \text{Store \VM{\verifier} as \VS{\verifier}} \\
 \pcln \label{enroll:fail} \text{Discard \VC{\pin}, \VC{\verifier}, \VC{\keyt_1}, \VC{\keyt_2}, \VC{\nonce}}, \tmp_{\VC{\counter}}, \tmp_{\VC{\state}} \< \<  \text{Discard \VS{\keyt_1}, \VS{\keyt_2}, \VS{\nonce}},  \tmp_{\VS{\counter}}, \tmp_{\VS{\state}} \\
 }
    \caption{Enrollment phase of authentication protocol}
    \label{fig:enrollment}
\end{figure}


==> introduction_copy.tex <==
%!TEX root = main.tex



\section{Introduction}



